Process Extraction from Text: Benchmarking the State of the Art and Paving the Way for Future Challenges

The extraction of process models from text refers to the problem of turning the information contained in an unstructured textual process descriptions into a formal representation,i.e.,a process model. Several automated approaches have been proposed to tackle this problem, but they are highly heterogeneous in scope and underlying assumptions,i.e., differences in input, target output, and data used in their evaluation.As a result, it is currently unclear how well existing solutions are able to solve the model-extraction problem and how they compare to each other.We overcome this issue by comparing 10 state-of-the-art approaches for model extraction in a systematic manner, covering both qualitative and quantitative aspects.The qualitative evaluation compares the analysis of the primary studies on: 1 the main characteristics of each solution;2 the type of process model elements extracted from the input data;3 the experimental evaluation performed to evaluate the proposed framework.The results show a heterogeneity of techniques, elements extracted and evaluations conducted, that are often impossible to compare.To overcome this difficulty we propose a quantitative comparison of the tools proposed by the papers on the unifying task of process model entity and relation extraction so as to be able to compare them directly.The results show three distinct groups of tools in terms of performance, with no tool obtaining very good scores and also serious limitations.Moreover, the proposed evaluation pipeline can be considered a reference task on a well-defined dataset and metrics that can be used to compare new tools. The paper also presents a reflection on the results of the qualitative and quantitative evaluation on the limitations and challenges that the community needs to address in the future to produce significant advances in this area.

==> sections/discussionqualitative.tex <==
%!TEX root = .././main.tex

\subsection*{Discussion of the Qualitative Comparative Analysis}
\label{sec:discussion-qualitative}
    
The analysis proposed in the previous Sections reveals several problematic aspects of state-of-the-art contributions. % in \pet. 
In this section, we elaborate on four sets of limitations %problematic questions 
concerning
\begin{enumerate*}[(i)]
	\item the data;
	\item to the techniques adopted;
	\item the experimental evaluation conducted; and 
	\item the pipeline proposed.
\end{enumerate*}

 %%%%%% DATA %%%%%%%%%%%%%%% 
\paragraph*{The data.}
\label{ssec:the-data}

A crucial set of limitations % questions 
concern the datasets adopted. 
Data are problematic in many ways:  
First of all, they are often not publicly available. 
Even worst, most of the available ones are somehow extracted from the dataset originally proposed in \citep{Friedrich11}. 
The only exception is the dataset proposed in \citep{DBLP:conf/caise/0003W0LLZLW20}. 
Nonetheless, we are doubtful of the usefulness of these data in addressing \pet challenges since it consists of instruction booklets and food recipes, whose complexity in terms of control flow is often simpler than the one of e.g., an administrative procedure.  
Second, the dataset in \citep{Friedrich11} presents some problematic aspects. A major problem is given by the fact that it is not representative of the variety of $<$process description, process diagram$>$ pairs one may have in real scenarios. 
%Having such a fully representative dataset may be too ambitious even for a high-quality dataset, given the variability of language and also the different ways in which the same intended process can be represented in a diagram. 
Nonetheless, the dataset in \citep{Friedrich11} was mainly the effort of a limited group of persons, missing the typical validation steps in the form of multiple annotations and inter-annotation agreements that are typically used to take care of the differences that may exist in human judgment.  
Third, this dataset represents pairs of process descriptions and process diagrams without any intermediate form of annotation. 
For example, the specific correspondence between a portion of the text and an activity, or a gateway, in the diagram is missing. 
As a consequence, the dataset is not ready to be used to work on and comparatively evaluate sub-tasks of \pet, such as e.g., activity (gateway, actor, or some specific relations among them) extraction from text. 
In our opinion, this lack of specific annotations had had a negative impact both on the investigation of specific sub-tasks of \pet, and on the development and the adoption of reference metrics to comparatively evaluate these specific sub-tasks. 
This contributed to creating the heterogeneous situation depicted in Table \ref{tab:experimental-evaluation}, where the different contributions can be hardly compared on common ground.
%
Fourth, the size of the datasets may be %is
 not large enough to support the training and testing required by many sophisticated machine-learning techniques. 
 We believe that this lack of good quality, large enough, publicly available annotated datasets, that reflect the real complexity of documents adopted in, e.g., companies or real organizations, is a core problem that is likely impeding the development of scalable proposals. 
 Such datasets could enable the adoption of recent \NLP~techniques and machine learning solutions to handle writing style variations and word ambiguities.
% 
%We believe that the BPM community, possibly adopting mechanisms similar to the ones that have made available dozens of event-logs via the BPI challenges (which, in turn, have had a crucial impact on the development of process mining from event-log techniques). In creating such datasets the community will have to answer some crucial questions such as \textit{how big a dataset should be? How varied should it be (both in terms of textual variability and process elements)? Do we need to focus on text annotated with specific elements or on pairs of textual fragments and their corresponding models? In this latter case, how do we deal with possibly equivalent models and the biases that may be introduced by providing only one process model?}

%%%

%%%%%% TECHNIQUES %%%%%%%%%%%%%%%
\paragraph{The techniques.}
\label{ssec:the-techniques}

The lack/availability of data has had a direct impact on the techniques that can be applied. % in \pet. 
In particular, the lack of big quantities of annotated data makes the training of neural models unfeasible and indeed most of the approaches resort to using rule-based strategies. 
Defining rules that are precise and general enough at the same time however appears to be problematic. Often word lists and external resources such as WordNet, and VerbNet are adopted to increase the coverage and robustness of generic rules (especially the ones that analyze SVO triples), but doing that makes the rules extremely tailored to specific scenarios,  writing styles, and formatting of documents with the result of having to refine/re-build the framework for each domain it is adopted in.
Another problem is related to the identification of activities, actors, and data-objects, via the analysis of verbs, and subject/object relations. An effective contribution of state-of-the-art works is that the analysis of SVO triples enables the differentiation between those verbs expressing activities and those verbs expressing events. 
Also, the extraction of the subject and the object of a verb allows the detection of actors and data-objects. 
However, almost all papers ignore the problem of false positives. 
This problem could be addressed using classifiers on top of the extraction mechanism, for example.
%Nonetheless, this would require annotated datasets containing also non-informative sentences (or more specifically here, sentences whose SVO triples do not almost always translate into an actor-activity-data object pattern).  
A further intriguing aspect of state-of-the-art contributions is that most works extract syntactic and semantic information through the analysis of the plain text and only a few papers provide a direct semantic representation of the text using semantic word embeddings. Given the impact that semantic word embeddings have recently had on different tasks in NLP, and the importance of it enhancing, e.g., the performance of statistical classifiers, this also opens interesting questions for future research efforts. 

All the problems above are somehow related and concern the usage of recent NLP advancements in \pet. While the usage of these techniques is related to the availability of data highlighted above, we also believe that this perspective puts forward interesting specific questions on the techniques adopted, such as: \textit{how can we leverage recent NLP advancements and increase the performance of \pet tasks? Can we adopt semantics embeddings to represent the input text instead of performing deep syntactical and semantical analyses with the available amount of data?} And ultimately, \textit{is it possible to build machine-learning-based techniques that overcome the current rule-based ones in terms of performance and generality?}

A final observation concerns the usage of external resources and NLP techniques/tools (such as coreference resolution tools) and in particular the lack of adoption of recent NLP techniques/tools, likely due to the lack of recent works on \pet. 
Given the recent advances in NLP, this observation raises an interesting question for the community: 
\textit{Can we increase the frameworks' performance by just leveraging recent NLP advancements and up-to-date resources?}
Answering this question would help in understanding which errors generated by State of the art approaches are due to the specific \pet techniques proposed, and which errors are due to obsolete NLP resources and instruments adopted.


%%%%%% EXPERIMENTAL EVALUATION %%%%%%%%%%%%%%%
\paragraph{The experimental evaluations.} 
\label{ssec:the-experimental-evaluations}

We have already discussed the problems related to the data, which influence also the experimental evaluations, and therefore we focus here on problems and challenges related to the metrics adopted to measure the performance of the proposed techniques.   

By looking at Table \ref{tab:experimental-evaluation} we can see that most contributions analyzed in this paper rely either on information retrieval measures or on graph-based measures. Nonetheless, the first problematic issue is that no real reference metrics exist in the community for the different proposed tasks. 
Another problem that should deserve some consideration is the fact that these metrics do not distinguish between possible kinds of errors that can be generated. For example, would it be better to identify a gateway but assign it to the wrong type or not identify it at all? Would it be better to associate the activity with the wrong actor or just to extract the activity? Answering these questions is a challenging task as extracting more information may help the manual refinement of the process, but errors that are not rectified may have significant negative consequences on the process model. 
A further problem is given by the fact that the metrics proposed in the literature mainly consider the graph structure of the process model and do not make a distinction between equivalent (very similar) process model fragments. As a very simple example, how should we evaluate when two activities are represented as compound activity in the diagram? 

Future work on \pet will also require addressing the challenges related to the metrics and in particular answering questions such as \textit{is it possible to propose reference metrics for the different specific subtasks of \pet as well as for the overall performance of the entire pipeline? Shall we distinguish among different types of errors or not? How do we take into account that different graph structures may convey the same (or very similar) semantic meanings?} The ultimate goal here would be to address two fundamental high-level questions: \textit{How can we measure the performance of a \pet framework? Which are the aspect of the framework we need to consider during an experimental evaluation?}  
  
%%%%%% PIPELINE %%%%%%%%%%%%%%%
\paragraph{The pipeline.}
\label{ssec:the-pipeline}

Concerning the overall pipeline, the analysis of the state-of-the-art contributions shows efforts in both the direct and the two-step approaches. While the direct approach may appear extremely attractive, due to the popularity of end-to-end machine learning approaches, the big question here is \textit{is there a way to collect the massive set of data that would require the construction of a generic direct pipeline?}  

If we focus on the two-step approach, we can identify a big potential advantage, because we can decompose the entire pipeline into modular subtasks and therefore work in a divide-et-impera manner, but also several problems and challenges. The first one relates to the composition of the pipeline, and to the different (sub)tasks in which we may decompose $\fa$ and $\fb$. As an example, we have noticed that the task of \textit{filtering out uninformative information} is rarely considered in state-of-the-art contributions but may be extremely important in real-world procedural documents. This could be due to the fact that there are almost no uninformative textual fragments in the reference dataset of \citet{Friedrich11} even though the pipeline should drive the construction of the datasets and not the other way around. Another challenge concerns the ordering of the different sub-tasks, and the impact it can have on the overall pipeline. For example, do we need to resolve coreferences before filtering out uninformative sentences from a text or can we postpone this task later? Another problematic aspect regards the labeling task and the available datasets for all the specific different su-tasks. As already mentioned when discussing the data problem, the reference dataset of \citet{Friedrich11} lacks an intermediate form of annotation and is therefore not directly usable for the construction and evaluation of e.g., a specific module dealing with the subtask of detecting noun-based activities. 
Further questions concern the usage of the intermediate representation. First of all, no clear reasons are given in papers on why a specific world model was used, and no study exists to assess whether some are better and offer a more robust intermediate representation. Second, sharing the data contained in different world models built by different \pet frameworks is currently very hard. This is extremely problematic, as having a common world model (or at least a way to move data across different ones) would boost a real modularization of $\fa$ and $\fb$, allowing reuse and the investigation of single components of the pipeline one at a time.

To sum up, the overall questions concerning the two-step approach are: \textit{can we provide a clear definition of the sub-tasks (or modules) that need to be performed to realize} $\fa$ \textit{and} $\fb$ \textit{and in which order they have to be composed? Can we support all the different modules with appropriate datasets? Is there a better world model in terms of robustness and efficient representation? Which are its characteristics? Can we define a common data structure to structure and share the intermediate representation?} And ultimately \textit{can the BPM community take advantage of the modular structure of the two-way approach to boost the research in \pet?}
    
    

==> sections/discussionquantitative.tex <==
%!TEX root = .././main.tex

\section*{Quantitative Discussion}
\label{sec:quantitative-discussion}
    
    
    

==> sections/experimentalsettings.tex <==
\subsection{Experimental settings}



==> sections/limitations.tex <==
%!TEX root = .././main.tex


\section{Limitations of the \SOTA} 
\label{sec:limitations}



==> sections/quantitative-metrics.tex <==
%!TEX root = .././main.tex



==> sections/quantitativestrictcomparison.tex <==
\subsection{Tools Comparisons} %Results of the Strict Comparison}
\label{ssec:results-strict-comparison}
%
\begin{table}[htb]
	\begin{center}
		\caption{The table reports the results of the strict comparison of the extraction of process elements from texts.}
		\label{tab:exact-match-elements}
	\end{center}
	\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccccccccccccc} 
    \toprule
    \multirow{3}{*}{\textbf{Paper}} & \multicolumn{3}{c}{\multirow{2}{*}{\textbf{Activity}}} & \multicolumn{3}{c}{\textbf{Activity}} & \multicolumn{3}{c}{\multirow{2}{*}{\textbf{Actor}}} & \multicolumn{3}{c}{\textbf{Further}} & \multicolumn{3}{c}{\textbf{XOR}} & \multicolumn{3}{c}{\textbf{Condition}} & \multicolumn{3}{c}{\textbf{AND}} \\
    %
    & & & & \multicolumn{3}{c}{\textbf{Data}} & & & &  \multicolumn{3}{c}{\textbf{Specification}} & \multicolumn{3}{c}{\textbf{Gateway}} & \multicolumn{3}{c}{\textbf{Specification}} & \multicolumn{3}{c}{\textbf{Gateway}} \\
    
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}  \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19} \cmidrule(lr){20-22}       
%
   & pr & rec & f1 & pr & rec & f1 & pr & rec & f1 & pr & rec & f1 & pr & rec & f1 & pr & rec & f1 & pr & rec & f1 \\
%  
\midrule 
\citet{derAaDiCiccio19} &
% Activity
0.08 & 0.13 & 0.10 & 
% Activity Data
0.00	 & 0.00 & 0.00 &  
% Actor
0.65 & 0.41 & 0.48 &  
- & - & - & 
- & - & - &  
- & - & - & 
- & - & - \\
%
\midrule  
\citet{GoncalvesSB11}&
%% Activity
0.42 & 0.32 & 0.35 & 
%% Activity Data
0.31 & 0.27 & 0.27 &  
%% Actor
0.59 & 0.31 & 0.39 & 
- & - & - &
- & - & - &  
- & - & - &  
- & - & - \\
%
\midrule  
\cite{Friedrich11} & 
% Activity 
0.56 & \textbf{0.77} & 0.64 &
% Activity Data 
0.38 & 0.48 & 0.41 &  
% Actor
0.66 & 0.63 & 0.63 &  
% Further Specification
0.17 & 0.27 & 0.19 & 
% XOR
0.50 & 0.26 & 0.32 & 
% Condition Specification
- & - & - & 
% And Gateway
\textbf{0.12} & \textbf{0.12} & \textbf{0.12} \\
%    
\midrule
\cite{EpureMHDS15}& 
%% Activity
0.12 & 0.15 & 0.13 & 
%% Activity Data  
0.02 & 0.04 & 0.03 & 
- & - & - &  - & - & - & - & - & - &  - & - & - &  - & - & - \\
%%     
\midrule
\citet{HonkiszK018} &
% Activity
\textbf{0.66} & 0.68 & \textbf{0.65} & 
% Activity Data
\textbf{0.02} & \textbf{0.03} & \textbf{0.03} &  
% Actor
\textbf{0.08} &\textbf{0.11} & \textbf{0.09} & 
% Further Spec.
 - & - & -  & 
 % XOR Gateway
\textbf{0.66} & \textbf{0.39} & \textbf{0.47} & 
% Condition Specification
0.11 & 0.08 & 0.09 & 
% AND 
 - & - & - \\
%
\midrule
\citet{DBLP:conf/caise/0003W0LLZLW20} &
% Activity
0.05 & 0.02 & 0.02 & 
% Activity Data
0.01 & 0.01 & 0.01 & 
% Actor
0.32 & 0.20 & 0.23 & 
 - & - & - &  - & - & - &  - & - & - &  - & - & - \\
    \bottomrule
    \end{tabular}
    }
\end{table}
%
%. RELATIONS
%
\begin{table}[htb]
	\begin{center}
		\caption{The table reports the results of the strict comparison of the extraction of process element relations from texts}
		\label{tab:exact-match-relations}
%		
	\end{center}
	\resizebox{\textwidth}{!}{\begin{tabular}{lcccccccccccccccccc} 
    \toprule
    \multirow{3}{*}{\textbf{Paper}} &\multicolumn{3}{c}{\multirow{2}{*}{\textbf{Uses}}} & \multicolumn{3}{c}{\textbf{Actor}} & \multicolumn{3}{c}{\textbf{Actor}} & \multicolumn{3}{c}{\textbf{Further}} & \multicolumn{3}{c}{\multirow{2}{*}{\textbf{Flow}}} & \multicolumn{3}{c}{\textbf{Same}}  \\
	%
     &&&& \multicolumn{3}{c}{\textbf{Performer}} & \multicolumn{3}{c}{\textbf{Recipient}} & \multicolumn{3}{c}{\textbf{Specification}} &&&& \multicolumn{3}{c}{\textbf{Gateway}}  \\
%
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}  \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}  
    %
    & pr & rec & f1 & pr & rec & f1 &pr & rec & f1 &pr & rec & f1 &pr & rec & f1 &pr & rec & f1 \\
% 
\midrule 
\citet{derAaDiCiccio19} & 
% Uses
0.00 & 0.00 & 0.00 & 
% Actor Performer
0.34 & 0.07 & 0.11 & 
% Actor Recipient
- & - & -  & 
% Further Spec.
- & - & -  & 
% Flow
- & - & -  & 
% Same Gateway
- & - & - \\
\midrule  
\citet{GoncalvesSB11} & 
% Uses
0.84 & 0.18 & 0.28 & 
% Actor-Performer
0.74 & 0.27 & 0.36 &  
% Actor Recipient
- & - & -  & 
% Further Spec.
- & - & -  & 
% Flow
0.51 & 0.05 & 0.09  & 
% Same Gateway
- & - & - \\
\midrule  
\cite{Friedrich11} & 
% Uses
\textbf{0.97} & \textbf{0.43} & \textbf{0.58} & 
% Actor-Performer
\textbf{0.97} & \textbf{0.69} & \textbf{0.78} & 
% Actor Recipient
- & - & -  & 
% Further Spec.
\textbf{0.56} & \textbf{0.27} & \textbf{0.35}  & 
% Flow
0.90 & 0.24 & 0.35  & 
% Same Gateway
- & - & - \\
\midrule
\cite{EpureMHDS15} & 
% Uses
0.12 & 0.01 & 0.02 & 
% Actor-Performer
- & - & - & 
% Actor Recipient
- & - & -  & 
% Further Spec.
- & - & -  & 
% Flow
0.23 & 0.01 & 0.03  & 
% Same Gateway
- & - & - \\
% 
\midrule
\citet{HonkiszK018} & 
% Uses
0.28 & 0.03 & 0.05 & 
% Actor-Performer
0.43 & 0.13 & 0.19 &  
% Actor Recipient
- & - & -  & 
% Further Spec.
- & - & -  & 
% Flow
\textbf{0.92} & \textbf{0.26} & \textbf{0.38}  & 
% Same Gateway
\textbf{0.07} & \textbf{0.07} & \textbf{0.07} \\
% 
\midrule
\citet{DBLP:conf/caise/0003W0LLZLW20} & 
% Uses
- & - & - & 
% Actor-Performer
- & - & - &  
% Actor Recipient
- & - & -  & 
% Further Spec.
- & - & -  & 
% Flow
- & - & -  & 
% Same Gateway
- & - & - \\
\bottomrule
    \end{tabular}
    }
	
\end{table}
%
%
In this section, we provide the results of the comparison of the tools when we compare the span of words extracted for the process elements with gold-standard annotations.
We report the results of process elements extraction in Table \ref{tab:exact-match-elements} and the results of process element relations extraction in Table \ref{tab:exact-match-relations}.

We start with the analysis of \textit{activity}.
This element is extracted by all the tools.
The most performing and precise tool is the one proposed by \citet{HonkiszK018}.
The tool of \citet{Friedrich11} has the highest recall, that is, it can extract most of the activities described in texts.
The tool of \citet{GoncalvesSB11} shows low performance, but it is still able to extract some activities.
The tools of \citet{derAaDiCiccio19, EpureMHDS15, DBLP:conf/caise/0003W0LLZLW20} have very low scores that provide their inability to extract \textit{activity} as defined in the PET annotation schema.
Also the object an activity acts on is extracted by all the tools.
Different from the situation depicted for activity extraction, the tool of \citet{HonkiszK018} shows severe difficulties to extract this element while the tool of \citet{Friedrich11} shows the best scores in all the three metrics.
The tool of \citet{GoncalvesSB11} is the second-best scoring tool. 
But, overall the scores for the extraction of this element are not satisfactory.
The tools of \citet{derAaDiCiccio19, EpureMHDS15, DBLP:conf/caise/0003W0LLZLW20} show very low scores. These demonstrate their inability to extract this element from texts.
The results of the \textit{uses} relation in Table \ref{tab:exact-match-relations} show the same situation for the extraction of \textit{activity data} element.
The tool of  \citet{Friedrich11} provides the highest scores in all three metrics. The tool of \citet{GoncalvesSB11} is the second-best scoring tool with good precision but low recall.
The other tools are not able to extract this element satisfactorily.

The extraction of \textit{actor} from text is performed in all the tools, but \citet{EpureMHDS15}.
The scores show that the most precise tools are the proposal of \citet{derAaDiCiccio19}, \citet{Friedrich11}, and \citet{GoncalvesSB11}.
The tool of  \citet{Friedrich11} reached the highest scores in all the metrics, while the tools of \citet{derAaDiCiccio19, GoncalvesSB11} show some difficulties in recalling all the actors mentioned in texts. 
The tools of \citet{HonkiszK018, DBLP:conf/caise/0003W0LLZLW20} are not able to provide any significant results.
The \textit{actor performer} relation is extracted by \citet{derAaDiCiccio19}, \citet{Friedrich11}, \citet{GoncalvesSB11}, and \citet{HonkiszK018}.
The scores reported in Table \ref{tab:exact-match-relations} show that the tool of \citet{Friedrich11} is the most performing tool.
It can correctly extract most of this relation from texts.
Indeed, it reached an almost perfect precision and a good recall.
In general, this tool provided satisfactory results for the extraction of the actors responsible for activities.
None of the tools directly extracted the \textit{actor recipient} relation in texts.
Only the tool of \citet{Friedrich11} captures the \textit{Further Specification} element and its relation with very low success.
Regarding this relation, we can say that further specification elements extracted are correctly linked to the activity they refer to, in many cases. 

Control flow structures are extracted by the tools of  \citet{Friedrich11, HonkiszK018} only.
Both the tools extract the \textit{XOR Gateway} element.
The one of \citet{HonkiszK018} performed slightly better in all three metrics.
The \textit{condition specification} element and the \textit{same gateway} relation are extracted by the tool of \citet{HonkiszK018} only, with very little success.
The \textit{AND Gateway} element is extracted by \citet{Friedrich11} only, with very little success.

Finally, the process model logic is extracted by extracting \textit{flow} relations among behavioral elements.
This relation is considered in the tools of \citet{EpureMHDS15, Friedrich11, GoncalvesSB11, HonkiszK018}.
Both tools have high precision, but low recall.
The most performant tool is the one of \citet{HonkiszK018} that has the highest scores in all the three metrics. 
Interestingly, the tool of \citet{Friedrich11} extracts slightly more activities from texts than the one of \citet{HonkiszK018}, but it is less efficient to extract control flow structures.
Since the xor gateway and condition specification elements play a direct role in extracting the overall process model logic, the tool of \citet{Friedrich11}reached the second-best scores.








==> sections/quantitativestrictcomparisonTables.tex <==
%!TEX root = ../main.tex

\section{Strict Comparisons of the Tools}

\begin{table}[tb]
	\begin{center}
		\caption{The table reports the results of the strict comparison of the extraction of process elements from texts.}
		\label{tab:exact-match-elements}
	\end{center}
	\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccccccccccccc} 
    \toprule
    \multirow{3}{*}{\textbf{Paper}} & \multicolumn{3}{c}{\multirow{2}{*}{\textbf{Activity}}} & \multicolumn{3}{c}{\textbf{Activity}} & \multicolumn{3}{c}{\multirow{2}{*}{\textbf{Actor}}} & \multicolumn{3}{c}{\textbf{Further}} & \multicolumn{3}{c}{\textbf{XOR}} & \multicolumn{3}{c}{\textbf{Condition}} & \multicolumn{3}{c}{\textbf{AND}} \\
    %
    & & & & \multicolumn{3}{c}{\textbf{Data}} & & & &  \multicolumn{3}{c}{\textbf{Specification}} & \multicolumn{3}{c}{\textbf{Gateway}} & \multicolumn{3}{c}{\textbf{Specification}} & \multicolumn{3}{c}{\textbf{Gateway}} \\
    
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}  \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19} \cmidrule(lr){20-22}       
%
   & pr & rec & f1 & pr & rec & f1 & pr & rec & f1 & pr & rec & f1 & pr & rec & f1 & pr & rec & f1 & pr & rec & f1 \\
%  
\midrule 
\citet{derAaDiCiccio19} &
% Activity
0.08 & 0.13 & 0.10 & 
% Activity Data
0.00	 & 0.00 & 0.00 &  
% Actor
0.65 & 0.41 & 0.48 &  
- & - & - & 
- & - & - &  
- & - & - & 
- & - & - \\
%
\midrule  
\citet{GoncalvesSB11}&
%% Activity
0.42 & 0.32 & 0.35 & 
%% Activity Data
0.31 & 0.27 & 0.27 &  
%% Actor
0.59 & 0.31 & 0.39 & 
- & - & - &
- & - & - &  
- & - & - &  
- & - & - \\
%
\midrule  
\cite{Friedrich11} & 
% Activity 
0.56 & \textbf{0.77} & 0.64 &
% Activity Data 
0.38 & 0.48 & 0.41 &  
% Actor
0.66 & 0.63 & 0.63 &  
% Further Specification
0.17 & 0.27 & 0.19 & 
% XOR
0.50 & 0.26 & 0.32 & 
% Condition Specification
- & - & - & 
% And Gateway
\textbf{0.12} & \textbf{0.12} & \textbf{0.12} \\
%    
\midrule
\cite{EpureMHDS15}& 
%% Activity
0.12 & 0.15 & 0.13 & 
%% Activity Data  
0.02 & 0.04 & 0.03 & 
- & - & - &  - & - & - & - & - & - &  - & - & - &  - & - & - \\
%%     
\midrule
\citet{HonkiszK018} &
% Activity
\textbf{0.66} & 0.68 & \textbf{0.65} & 
% Activity Data
\textbf{0.02} & \textbf{0.03} & \textbf{0.03} &  
% Actor
\textbf{0.08} &\textbf{0.11} & \textbf{0.09} & 
% Further Spec.
 - & - & -  & 
 % XOR Gateway
\textbf{0.66} & \textbf{0.39} & \textbf{0.47} & 
% Condition Specification
0.11 & 0.08 & 0.09 & 
% AND 
 - & - & - \\
%
\midrule
\citet{DBLP:conf/caise/0003W0LLZLW20} &
% Activity
0.05 & 0.02 & 0.02 & 
% Activity Data
0.01 & 0.01 & 0.01 & 
% Actor
0.32 & 0.20 & 0.23 & 
 - & - & - &  - & - & - &  - & - & - &  - & - & - \\
    \bottomrule
    \end{tabular}
    }
\end{table}
%
%. RELATIONS
%
\begin{table}[htb]
	\begin{center}
		\caption{The table reports the results of the strict comparison of the extraction of process element relations from texts}
		\label{tab:exact-match-relations}
%		
	\end{center}
	\resizebox{\textwidth}{!}{\begin{tabular}{lcccccccccccccccccc} 
    \toprule
    \multirow{3}{*}{\textbf{Paper}} &\multicolumn{3}{c}{\multirow{2}{*}{\textbf{Uses}}} & \multicolumn{3}{c}{\textbf{Actor}} & \multicolumn{3}{c}{\textbf{Actor}} & \multicolumn{3}{c}{\textbf{Further}} & \multicolumn{3}{c}{\multirow{2}{*}{\textbf{Flow}}} & \multicolumn{3}{c}{\textbf{Same}}  \\
	%
     &&&& \multicolumn{3}{c}{\textbf{Performer}} & \multicolumn{3}{c}{\textbf{Recipient}} & \multicolumn{3}{c}{\textbf{Specification}} &&&& \multicolumn{3}{c}{\textbf{Gateway}}  \\
%
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}  \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}  
    %
    & pr & rec & f1 & pr & rec & f1 &pr & rec & f1 &pr & rec & f1 &pr & rec & f1 &pr & rec & f1 \\
% 
\midrule 
\citet{derAaDiCiccio19} & 
% Uses
0.00 & 0.00 & 0.00 & 
% Actor Performer
0.34 & 0.07 & 0.11 & 
% Actor Recipient
- & - & -  & 
% Further Spec.
- & - & -  & 
% Flow
- & - & -  & 
% Same Gateway
- & - & - \\
\midrule  
\citet{GoncalvesSB11} & 
% Uses
0.84 & 0.18 & 0.28 & 
% Actor-Performer
0.74 & 0.27 & 0.36 &  
% Actor Recipient
- & - & -  & 
% Further Spec.
- & - & -  & 
% Flow
0.51 & 0.05 & 0.09  & 
% Same Gateway
- & - & - \\
\midrule  
\cite{Friedrich11} & 
% Uses
\textbf{0.97} & \textbf{0.43} & \textbf{0.58} & 
% Actor-Performer
\textbf{0.97} & \textbf{0.69} & \textbf{0.78} & 
% Actor Recipient
- & - & -  & 
% Further Spec.
\textbf{0.56} & \textbf{0.27} & \textbf{0.35}  & 
% Flow
0.90 & 0.24 & 0.35  & 
% Same Gateway
- & - & - \\
\midrule
\cite{EpureMHDS15} & 
% Uses
0.12 & 0.01 & 0.02 & 
% Actor-Performer
- & - & - & 
% Actor Recipient
- & - & -  & 
% Further Spec.
- & - & -  & 
% Flow
0.23 & 0.01 & 0.03  & 
% Same Gateway
- & - & - \\
% 
\midrule
\citet{HonkiszK018} & 
% Uses
0.28 & 0.03 & 0.05 & 
% Actor-Performer
0.43 & 0.13 & 0.19 &  
% Actor Recipient
- & - & -  & 
% Further Spec.
- & - & -  & 
% Flow
\textbf{0.92} & \textbf{0.26} & \textbf{0.38}  & 
% Same Gateway
\textbf{0.07} & \textbf{0.07} & \textbf{0.07} \\
% 
\midrule
\citet{DBLP:conf/caise/0003W0LLZLW20} & 
% Uses
- & - & - & 
% Actor-Performer
- & - & - &  
% Actor Recipient
- & - & -  & 
% Further Spec.
- & - & -  & 
% Flow
- & - & -  & 
% Same Gateway
- & - & - \\
\bottomrule
    \end{tabular}
    }
	
\end{table}
%
%%
%In this section, we provide the results of the comparison of the tools when we compare the span of words extracted for the process elements with gold-standard annotations.
%We report the results of process elements extraction in Table \ref{tab:exact-match-elements} and the results of process element relations extraction in Table \ref{tab:exact-match-relations}.
%
%We start with the analysis of \textit{activity}.
%This element is extracted by all the tools.
%The most performing and precise tool is the one proposed by \citet{HonkiszK018}.
%The tool of \citet{Friedrich11} has the highest recall, that is, it can extract most of the activities described in texts.
%The tool of \citet{GoncalvesSB11} shows low performance, but it is still able to extract some activities.
%The tools of \citet{derAaDiCiccio19, EpureMHDS15, DBLP:conf/caise/0003W0LLZLW20} have very low scores that provide their inability to extract \textit{activity} as defined in the PET annotation schema.
%Also the object an activity acts on is extracted by all the tools.
%Different from the situation depicted for activity extraction, the tool of \citet{HonkiszK018} shows severe difficulties to extract this element while the tool of \citet{Friedrich11} shows the best scores in all the three metrics.
%The tool of \citet{GoncalvesSB11} is the second-best scoring tool. 
%But, overall the scores for the extraction of this element are not satisfactory.
%The tools of \citet{derAaDiCiccio19, EpureMHDS15, DBLP:conf/caise/0003W0LLZLW20} show very low scores. These demonstrate their inability to extract this element from texts.
%The results of the \textit{uses} relation in Table \ref{tab:exact-match-relations} show the same situation for the extraction of \textit{activity data} element.
%The tool of  \citet{Friedrich11} provides the highest scores in all three metrics. The tool of \citet{GoncalvesSB11} is the second-best scoring tool with good precision but low recall.
%The other tools are not able to extract this element satisfactorily.
%
%The extraction of \textit{actor} from text is performed in all the tools, but \citet{EpureMHDS15}.
%The scores show that the most precise tools are the proposal of \citet{derAaDiCiccio19}, \citet{Friedrich11}, and \citet{GoncalvesSB11}.
%The tool of  \citet{Friedrich11} reached the highest scores in all the metrics, while the tools of \citet{derAaDiCiccio19, GoncalvesSB11} show some difficulties in recalling all the actors mentioned in texts. 
%The tools of \citet{HonkiszK018, DBLP:conf/caise/0003W0LLZLW20} are not able to provide any significant results.
%The \textit{actor performer} relation is extracted by \citet{derAaDiCiccio19}, \citet{Friedrich11}, \citet{GoncalvesSB11}, and \citet{HonkiszK018}.
%The scores reported in Table \ref{tab:exact-match-relations} show that the tool of \citet{Friedrich11} is the most performing tool.
%It can correctly extract most of this relation from texts.
%Indeed, it reached an almost perfect precision and a good recall.
%In general, this tool provided satisfactory results for the extraction of the actors responsible for activities.
%None of the tools directly extracted the \textit{actor recipient} relation in texts.
%Only the tool of \citet{Friedrich11} captures the \textit{Further Specification} element and its relation with very low success.
%Regarding this relation, we can say that further specification elements extracted are correctly linked to the activity they refer to, in many cases. 
%
%Control flow structures are extracted by the tools of  \citet{Friedrich11, HonkiszK018} only.
%Both the tools extract the \textit{XOR Gateway} element.
%The one of \citet{HonkiszK018} performed slightly better in all three metrics.
%The \textit{condition specification} element and the \textit{same gateway} relation are extracted by the tool of \citet{HonkiszK018} only, with very little success.
%The \textit{AND Gateway} element is extracted by \citet{Friedrich11} only, with very little success.
%
%Finally, the process model logic is extracted by extracting \textit{flow} relations among behavioral elements.
%This relation is considered in the tools of \citet{EpureMHDS15, Friedrich11, GoncalvesSB11, HonkiszK018}.
%Both tools have high precision, but low recall.
%The most performant tool is the one of \citet{HonkiszK018} that has the highest scores in all the three metrics. 
%Interestingly, the tool of \citet{Friedrich11} extracts slightly more activities from texts than the one of \citet{HonkiszK018}, but it is less efficient to extract control flow structures.
%Since the xor gateway and condition specification elements play a direct role in extracting the overall process model logic, the tool of \citet{Friedrich11}reached the second-best scores.
%
%
%





==> sections/table-elements-old-backup.tex <==
\begin{table*}[hbt!] % {tab:process-elements}
	\renewcommand{\arraystretch}{1.2}
    \begin{center}
     \caption{Elements extracted from the input text.}
     \label{tab:process-elements}
    \begin{tabular}{lcccccc} %\begin{tabular}{l|ccc|ccccc}
    \toprule
    & & \multicolumn{3}{c}{Control Fow} &  \multicolumn{2}{c}{Participant} \\ 
	\cmidrule(lr){3-5}\cmidrule(lr){6-7}
    Paper &  Approach & Activity & Event & Gateway & Actor & Artifact \\ 
   \midrule
	\citet{AckermannV13} & \multirow{4}{*}{$f$} & \yes & \yes & \yes & \yes & \yes \\
	\citet{derAaDiCiccio19} & &\yes & \no & \no & \no & \no \\
	\citet{DBLP:conf/caise/LopezSNM21} & & \yes & \no & \yes & \no & \no \\
	\citet{Han2020} & & \yes & \yes & \yes & \no & \no \\ 
	\arrayrulecolor{gray}
	\cmidrule{2-7}
	\citet{GoncalvesSB11} & \multirow{5}{*}{$\fa \circ \fb$} & \yes & \yes & \yes & \yes & \yes \\
	\citet{SawantRSPS14} & & \yes & \yes & \yes & \yes & \yes \\
	\citet{Friedrich11}  & & \yes & \yes & \yes & \yes & \yes \\
	\citet{EpureMHDS15} & & \yes & \no & \yes & \yes & \no \\ 
	\citet{HonkiszK018} & & \yes & \yes & \yes & \no & \yes \\ 
	\arrayrulecolor{gray}
	\cmidrule{2-7}
	\citet{Ferreira17} & \multirow{4}{*}{$f_a$} & \yes & \yes & \yes & \no & \yes \\
	\citet{DBLP:conf/caise/0003W0LLZLW20} & & \yes & \no & \no & \yes & \yes \\ 
	\citet{DBLP:conf/bpm/QuishpiCP20} & & \yes & \yes & \yes & \yes & \yes \\
	\citet{Leopold18} & & \yes & \no & \no & \yes & \no \\
    \bottomrule
    \end{tabular}
    \end{center}
\end{table*}
